A hyperbolicity-preserving discontinuous stochastic Galerkin scheme for uncertain hyperbolic systems of equations

Intrusive Uncertainty Quantification methods such as stochastic Galerkin are gaining popularity, whereas the classical stochastic Galerkin approach is not ensured to preserve hyperbolicity of the underlying hyperbolic system. We apply a modification of this method that uses a slope limiter to retain admissible solutions of the system, while providing high-order approximations in the physical and stochastic space. This is done using a spatial discontinuous Galerkin scheme and a Multi-Element stochastic Galerkin ansatz in the random space. We analyze the convergence of the resulting scheme and apply it to the compressible Euler equations with various uncertain initial states in one and two spatial domains with up to three uncertainties. The performance in multiple stochastic dimensions is compared to the non-intrusive Stochastic Collocation method. The numerical results underline the strength of our method, especially if discontinuities are present in the uncertainty of the solution.

==> Images/cbtest.tex <==
\def\mycolormap{                rgb(0pt)=(0,0,0.5625);
                rgb(1pt)=(0,0,0.625);
                rgb(2pt)=(0,0,0.6875);
                rgb(3pt)=(0,0,0.75);
                rgb(4pt)=(0,0,0.8125);
                rgb(5pt)=(0,0,0.875);
                rgb(6pt)=(0,0,0.9375);
                rgb(7pt)=(0,0,1);
                rgb(8pt)=(0,0.0625,1);
                rgb(9pt)=(0,0.125,1);
                rgb(10pt)=(0,0.1875,1);
                rgb(11pt)=(0,0.25,1);
                rgb(12pt)=(0,0.3125,1);
                rgb(13pt)=(0,0.375,1);
                rgb(14pt)=(0,0.4375,1);
                rgb(15pt)=(0,0.5,1);
                rgb(16pt)=(0,0.5625,1);
                rgb(17pt)=(0,0.625,1);
                rgb(18pt)=(0,0.6875,1);
                rgb(19pt)=(0,0.75,1);
                rgb(20pt)=(0,0.8125,1);
                rgb(21pt)=(0,0.875,1);
                rgb(22pt)=(0,0.9375,1);
                rgb(23pt)=(0,1,1);
                rgb(24pt)=(0.0625,1,0.9375);
                rgb(25pt)=(0.125,1,0.875);
                rgb(26pt)=(0.1875,1,0.8125);
                rgb(27pt)=(0.25,1,0.75);
                rgb(28pt)=(0.3125,1,0.6875);
                rgb(29pt)=(0.375,1,0.625);
                rgb(30pt)=(0.4375,1,0.5625);
                rgb(31pt)=(0.5,1,0.5);
                rgb(32pt)=(0.5625,1,0.4375);
                rgb(33pt)=(0.625,1,0.375);
                rgb(34pt)=(0.6875,1,0.3125);
                rgb(35pt)=(0.75,1,0.25);
                rgb(36pt)=(0.8125,1,0.1875);
                rgb(37pt)=(0.875,1,0.125);
                rgb(38pt)=(0.9375,1,0.0625);
                rgb(39pt)=(1,1,0);
                rgb(40pt)=(1,0.9375,0);
                rgb(41pt)=(1,0.875,0);
                rgb(42pt)=(1,0.8125,0);
                rgb(43pt)=(1,0.75,0);
                rgb(44pt)=(1,0.6875,0);
                rgb(45pt)=(1,0.625,0);
                rgb(46pt)=(1,0.5625,0);
                rgb(47pt)=(1,0.5,0);
                rgb(48pt)=(1,0.4375,0);
                rgb(49pt)=(1,0.375,0);
                rgb(50pt)=(1,0.3125,0);
                rgb(51pt)=(1,0.25,0);
                rgb(52pt)=(1,0.1875,0);
                rgb(53pt)=(1,0.125,0);
                rgb(54pt)=(1,0.0625,0);
                rgb(55pt)=(1,0,0);
                rgb(56pt)=(0.9375,0,0);
                rgb(57pt)=(0.875,0,0);
                rgb(58pt)=(0.8125,0,0);
                rgb(59pt)=(0.75,0,0);
                rgb(60pt)=(0.6875,0,0);
                rgb(61pt)=(0.625,0,0);
                rgb(62pt)=(0.5625,0,0);
                rgb(63pt)=(0.5,0,0)}

==> Images/colormap_jet.tex <==
\pgfplotsset{colormap={jet}{[1pt]
rgb(0pt)=(0.500000,0.000000,0.000000);
rgb(1pt)=(0.504000,0.000000,0.000000);
rgb(2pt)=(0.508000,0.000000,0.000000);
rgb(3pt)=(0.512000,0.000000,0.000000);
rgb(4pt)=(0.516000,0.000000,0.000000);
rgb(5pt)=(0.520000,0.000000,0.000000);
rgb(6pt)=(0.524000,0.000000,0.000000);
rgb(7pt)=(0.528000,0.000000,0.000000);
rgb(8pt)=(0.532000,0.000000,0.000000);
rgb(9pt)=(0.536000,0.000000,0.000000);
rgb(10pt)=(0.540000,0.000000,0.000000);
rgb(11pt)=(0.544000,0.000000,0.000000);
rgb(12pt)=(0.548000,0.000000,0.000000);
rgb(13pt)=(0.552000,0.000000,0.000000);
rgb(14pt)=(0.556000,0.000000,0.000000);
rgb(15pt)=(0.560000,0.000000,0.000000);
rgb(16pt)=(0.564000,0.000000,0.000000);
rgb(17pt)=(0.568000,0.000000,0.000000);
rgb(18pt)=(0.572000,0.000000,0.000000);
rgb(19pt)=(0.576000,0.000000,0.000000);
rgb(20pt)=(0.580000,0.000000,0.000000);
rgb(21pt)=(0.584000,0.000000,0.000000);
rgb(22pt)=(0.588000,0.000000,0.000000);
rgb(23pt)=(0.592000,0.000000,0.000000);
rgb(24pt)=(0.596000,0.000000,0.000000);
rgb(25pt)=(0.600000,0.000000,0.000000);
rgb(26pt)=(0.604000,0.000000,0.000000);
rgb(27pt)=(0.608000,0.000000,0.000000);
rgb(28pt)=(0.612000,0.000000,0.000000);
rgb(29pt)=(0.616000,0.000000,0.000000);
rgb(30pt)=(0.620000,0.000000,0.000000);
rgb(31pt)=(0.624000,0.000000,0.000000);
rgb(32pt)=(0.628000,0.000000,0.000000);
rgb(33pt)=(0.632000,0.000000,0.000000);
rgb(34pt)=(0.636000,0.000000,0.000000);
rgb(35pt)=(0.640000,0.000000,0.000000);
rgb(36pt)=(0.644000,0.000000,0.000000);
rgb(37pt)=(0.648000,0.000000,0.000000);
rgb(38pt)=(0.652000,0.000000,0.000000);
rgb(39pt)=(0.656000,0.000000,0.000000);
rgb(40pt)=(0.660000,0.000000,0.000000);
rgb(41pt)=(0.664000,0.000000,0.000000);
rgb(42pt)=(0.668000,0.000000,0.000000);
rgb(43pt)=(0.672000,0.000000,0.000000);
rgb(44pt)=(0.676000,0.000000,0.000000);
rgb(45pt)=(0.680000,0.000000,0.000000);
rgb(46pt)=(0.684000,0.000000,0.000000);
rgb(47pt)=(0.688000,0.000000,0.000000);
rgb(48pt)=(0.692000,0.000000,0.000000);
rgb(49pt)=(0.696000,0.000000,0.000000);
rgb(50pt)=(0.700000,0.000000,0.000000);
rgb(51pt)=(0.704000,0.000000,0.000000);
rgb(52pt)=(0.708000,0.000000,0.000000);
rgb(53pt)=(0.712000,0.000000,0.000000);
rgb(54pt)=(0.716000,0.000000,0.000000);
rgb(55pt)=(0.720000,0.000000,0.000000);
rgb(56pt)=(0.724000,0.000000,0.000000);
rgb(57pt)=(0.728000,0.000000,0.000000);
rgb(58pt)=(0.732000,0.000000,0.000000);
rgb(59pt)=(0.736000,0.000000,0.000000);
rgb(60pt)=(0.740000,0.000000,0.000000);
rgb(61pt)=(0.744000,0.000000,0.000000);
rgb(62pt)=(0.748000,0.000000,0.000000);
rgb(63pt)=(0.752000,0.000000,0.000000);
rgb(64pt)=(0.756000,0.000000,0.000000);
rgb(65pt)=(0.760000,0.000000,0.000000);
rgb(66pt)=(0.764000,0.000000,0.000000);
rgb(67pt)=(0.768000,0.000000,0.000000);
rgb(68pt)=(0.772000,0.000000,0.000000);
rgb(69pt)=(0.776000,0.000000,0.000000);
rgb(70pt)=(0.780000,0.000000,0.000000);
rgb(71pt)=(0.784000,0.000000,0.000000);
rgb(72pt)=(0.788000,0.000000,0.000000);
rgb(73pt)=(0.792000,0.000000,0.000000);
rgb(74pt)=(0.796000,0.000000,0.000000);
rgb(75pt)=(0.800000,0.000000,0.000000);
rgb(76pt)=(0.804000,0.000000,0.000000);
rgb(77pt)=(0.808000,0.000000,0.000000);
rgb(78pt)=(0.812000,0.000000,0.000000);
rgb(79pt)=(0.816000,0.000000,0.000000);
rgb(80pt)=(0.820000,0.000000,0.000000);
rgb(81pt)=(0.824000,0.000000,0.000000);
rgb(82pt)=(0.828000,0.000000,0.000000);
rgb(83pt)=(0.832000,0.000000,0.000000);
rgb(84pt)=(0.836000,0.000000,0.000000);
rgb(85pt)=(0.840000,0.000000,0.000000);
rgb(86pt)=(0.844000,0.000000,0.000000);
rgb(87pt)=(0.848000,0.000000,0.000000);
rgb(88pt)=(0.852000,0.000000,0.000000);
rgb(89pt)=(0.856000,0.000000,0.000000);
rgb(90pt)=(0.860000,0.000000,0.000000);
rgb(91pt)=(0.864000,0.000000,0.000000);
rgb(92pt)=(0.868000,0.000000,0.000000);
rgb(93pt)=(0.872000,0.000000,0.000000);
rgb(94pt)=(0.876000,0.000000,0.000000);
rgb(95pt)=(0.880000,0.000000,0.000000);
rgb(96pt)=(0.884000,0.000000,0.000000);
rgb(97pt)=(0.888000,0.000000,0.000000);
rgb(98pt)=(0.892000,0.000000,0.000000);
rgb(99pt)=(0.896000,0.000000,0.000000);
rgb(100pt)=(0.900000,0.000000,0.000000);
rgb(101pt)=(0.904000,0.000000,0.000000);
rgb(102pt)=(0.908000,0.000000,0.000000);
rgb(103pt)=(0.912000,0.000000,0.000000);
rgb(104pt)=(0.916000,0.000000,0.000000);
rgb(105pt)=(0.920000,0.000000,0.000000);
rgb(106pt)=(0.924000,0.000000,0.000000);
rgb(107pt)=(0.928000,0.000000,0.000000);
rgb(108pt)=(0.932000,0.000000,0.000000);
rgb(109pt)=(0.936000,0.000000,0.000000);
rgb(110pt)=(0.940000,0.000000,0.000000);
rgb(111pt)=(0.944000,0.000000,0.000000);
rgb(112pt)=(0.948000,0.000000,0.000000);
rgb(113pt)=(0.952000,0.000000,0.000000);
rgb(114pt)=(0.956000,0.000000,0.000000);
rgb(115pt)=(0.960000,0.000000,0.000000);
rgb(116pt)=(0.964000,0.000000,0.000000);
rgb(117pt)=(0.968000,0.000000,0.000000);
rgb(118pt)=(0.972000,0.000000,0.000000);
rgb(119pt)=(0.976000,0.000000,0.000000);
rgb(120pt)=(0.980000,0.000000,0.000000);
rgb(121pt)=(0.984000,0.000000,0.000000);
rgb(122pt)=(0.988000,0.000000,0.000000);
rgb(123pt)=(0.992000,0.000000,0.000000);
rgb(124pt)=(0.996000,0.000000,0.000000);
rgb(125pt)=(1.000000,0.000000,0.000000);
rgb(126pt)=(1.000000,0.004000,0.000000);
rgb(127pt)=(1.000000,0.008000,0.000000);
rgb(128pt)=(1.000000,0.012000,0.000000);
rgb(129pt)=(1.000000,0.016000,0.000000);
rgb(130pt)=(1.000000,0.020000,0.000000);
rgb(131pt)=(1.000000,0.024000,0.000000);
rgb(132pt)=(1.000000,0.028000,0.000000);
rgb(133pt)=(1.000000,0.032000,0.000000);
rgb(134pt)=(1.000000,0.036000,0.000000);
rgb(135pt)=(1.000000,0.040000,0.000000);
rgb(136pt)=(1.000000,0.044000,0.000000);
rgb(137pt)=(1.000000,0.048000,0.000000);
rgb(138pt)=(1.000000,0.052000,0.000000);
rgb(139pt)=(1.000000,0.056000,0.000000);
rgb(140pt)=(1.000000,0.060000,0.000000);
rgb(141pt)=(1.000000,0.064000,0.000000);
rgb(142pt)=(1.000000,0.068000,0.000000);
rgb(143pt)=(1.000000,0.072000,0.000000);
rgb(144pt)=(1.000000,0.076000,0.000000);
rgb(145pt)=(1.000000,0.080000,0.000000);
rgb(146pt)=(1.000000,0.084000,0.000000);
rgb(147pt)=(1.000000,0.088000,0.000000);
rgb(148pt)=(1.000000,0.092000,0.000000);
rgb(149pt)=(1.000000,0.096000,0.000000);
rgb(150pt)=(1.000000,0.100000,0.000000);
rgb(151pt)=(1.000000,0.104000,0.000000);
rgb(152pt)=(1.000000,0.108000,0.000000);
rgb(153pt)=(1.000000,0.112000,0.000000);
rgb(154pt)=(1.000000,0.116000,0.000000);
rgb(155pt)=(1.000000,0.120000,0.000000);
rgb(156pt)=(1.000000,0.124000,0.000000);
rgb(157pt)=(1.000000,0.128000,0.000000);
rgb(158pt)=(1.000000,0.132000,0.000000);
rgb(159pt)=(1.000000,0.136000,0.000000);
rgb(160pt)=(1.000000,0.140000,0.000000);
rgb(161pt)=(1.000000,0.144000,0.000000);
rgb(162pt)=(1.000000,0.148000,0.000000);
rgb(163pt)=(1.000000,0.152000,0.000000);
rgb(164pt)=(1.000000,0.156000,0.000000);
rgb(165pt)=(1.000000,0.160000,0.000000);
rgb(166pt)=(1.000000,0.164000,0.000000);
rgb(167pt)=(1.000000,0.168000,0.000000);
rgb(168pt)=(1.000000,0.172000,0.000000);
rgb(169pt)=(1.000000,0.176000,0.000000);
rgb(170pt)=(1.000000,0.180000,0.000000);
rgb(171pt)=(1.000000,0.184000,0.000000);
rgb(172pt)=(1.000000,0.188000,0.000000);
rgb(173pt)=(1.000000,0.192000,0.000000);
rgb(174pt)=(1.000000,0.196000,0.000000);
rgb(175pt)=(1.000000,0.200000,0.000000);
rgb(176pt)=(1.000000,0.204000,0.000000);
rgb(177pt)=(1.000000,0.208000,0.000000);
rgb(178pt)=(1.000000,0.212000,0.000000);
rgb(179pt)=(1.000000,0.216000,0.000000);
rgb(180pt)=(1.000000,0.220000,0.000000);
rgb(181pt)=(1.000000,0.224000,0.000000);
rgb(182pt)=(1.000000,0.228000,0.000000);
rgb(183pt)=(1.000000,0.232000,0.000000);
rgb(184pt)=(1.000000,0.236000,0.000000);
rgb(185pt)=(1.000000,0.240000,0.000000);
rgb(186pt)=(1.000000,0.244000,0.000000);
rgb(187pt)=(1.000000,0.248000,0.000000);
rgb(188pt)=(1.000000,0.252000,0.000000);
rgb(189pt)=(1.000000,0.256000,0.000000);
rgb(190pt)=(1.000000,0.260000,0.000000);
rgb(191pt)=(1.000000,0.264000,0.000000);
rgb(192pt)=(1.000000,0.268000,0.000000);
rgb(193pt)=(1.000000,0.272000,0.000000);
rgb(194pt)=(1.000000,0.276000,0.000000);
rgb(195pt)=(1.000000,0.280000,0.000000);
rgb(196pt)=(1.000000,0.284000,0.000000);
rgb(197pt)=(1.000000,0.288000,0.000000);
rgb(198pt)=(1.000000,0.292000,0.000000);
rgb(199pt)=(1.000000,0.296000,0.000000);
rgb(200pt)=(1.000000,0.300000,0.000000);
rgb(201pt)=(1.000000,0.304000,0.000000);
rgb(202pt)=(1.000000,0.308000,0.000000);
rgb(203pt)=(1.000000,0.312000,0.000000);
rgb(204pt)=(1.000000,0.316000,0.000000);
rgb(205pt)=(1.000000,0.320000,0.000000);
rgb(206pt)=(1.000000,0.324000,0.000000);
rgb(207pt)=(1.000000,0.328000,0.000000);
rgb(208pt)=(1.000000,0.332000,0.000000);
rgb(209pt)=(1.000000,0.336000,0.000000);
rgb(210pt)=(1.000000,0.340000,0.000000);
rgb(211pt)=(1.000000,0.344000,0.000000);
rgb(212pt)=(1.000000,0.348000,0.000000);
rgb(213pt)=(1.000000,0.352000,0.000000);
rgb(214pt)=(1.000000,0.356000,0.000000);
rgb(215pt)=(1.000000,0.360000,0.000000);
rgb(216pt)=(1.000000,0.364000,0.000000);
rgb(217pt)=(1.000000,0.368000,0.000000);
rgb(218pt)=(1.000000,0.372000,0.000000);
rgb(219pt)=(1.000000,0.376000,0.000000);
rgb(220pt)=(1.000000,0.380000,0.000000);
rgb(221pt)=(1.000000,0.384000,0.000000);
rgb(222pt)=(1.000000,0.388000,0.000000);
rgb(223pt)=(1.000000,0.392000,0.000000);
rgb(224pt)=(1.000000,0.396000,0.000000);
rgb(225pt)=(1.000000,0.400000,0.000000);
rgb(226pt)=(1.000000,0.404000,0.000000);
rgb(227pt)=(1.000000,0.408000,0.000000);
rgb(228pt)=(1.000000,0.412000,0.000000);
rgb(229pt)=(1.000000,0.416000,0.000000);
rgb(230pt)=(1.000000,0.420000,0.000000);
rgb(231pt)=(1.000000,0.424000,0.000000);
rgb(232pt)=(1.000000,0.428000,0.000000);
rgb(233pt)=(1.000000,0.432000,0.000000);
rgb(234pt)=(1.000000,0.436000,0.000000);
rgb(235pt)=(1.000000,0.440000,0.000000);
rgb(236pt)=(1.000000,0.444000,0.000000);
rgb(237pt)=(1.000000,0.448000,0.000000);
rgb(238pt)=(1.000000,0.452000,0.000000);
rgb(239pt)=(1.000000,0.456000,0.000000);
rgb(240pt)=(1.000000,0.460000,0.000000);
rgb(241pt)=(1.000000,0.464000,0.000000);
rgb(242pt)=(1.000000,0.468000,0.000000);
rgb(243pt)=(1.000000,0.472000,0.000000);
rgb(244pt)=(1.000000,0.476000,0.000000);
rgb(245pt)=(1.000000,0.480000,0.000000);
rgb(246pt)=(1.000000,0.484000,0.000000);
rgb(247pt)=(1.000000,0.488000,0.000000);
rgb(248pt)=(1.000000,0.492000,0.000000);
rgb(249pt)=(1.000000,0.496000,0.000000);
rgb(250pt)=(1.000000,0.500000,0.000000);
rgb(251pt)=(1.000000,0.504000,0.000000);
rgb(252pt)=(1.000000,0.508000,0.000000);
rgb(253pt)=(1.000000,0.512000,0.000000);
rgb(254pt)=(1.000000,0.516000,0.000000);
rgb(255pt)=(1.000000,0.520000,0.000000);
rgb(256pt)=(1.000000,0.524000,0.000000);
rgb(257pt)=(1.000000,0.528000,0.000000);
rgb(258pt)=(1.000000,0.532000,0.000000);
rgb(259pt)=(1.000000,0.536000,0.000000);
rgb(260pt)=(1.000000,0.540000,0.000000);
rgb(261pt)=(1.000000,0.544000,0.000000);
rgb(262pt)=(1.000000,0.548000,0.000000);
rgb(263pt)=(1.000000,0.552000,0.000000);
rgb(264pt)=(1.000000,0.556000,0.000000);
rgb(265pt)=(1.000000,0.560000,0.000000);
rgb(266pt)=(1.000000,0.564000,0.000000);
rgb(267pt)=(1.000000,0.568000,0.000000);
rgb(268pt)=(1.000000,0.572000,0.000000);
rgb(269pt)=(1.000000,0.576000,0.000000);
rgb(270pt)=(1.000000,0.580000,0.000000);
rgb(271pt)=(1.000000,0.584000,0.000000);
rgb(272pt)=(1.000000,0.588000,0.000000);
rgb(273pt)=(1.000000,0.592000,0.000000);
rgb(274pt)=(1.000000,0.596000,0.000000);
rgb(275pt)=(1.000000,0.600000,0.000000);
rgb(276pt)=(1.000000,0.604000,0.000000);
rgb(277pt)=(1.000000,0.608000,0.000000);
rgb(278pt)=(1.000000,0.612000,0.000000);
rgb(279pt)=(1.000000,0.616000,0.000000);
rgb(280pt)=(1.000000,0.620000,0.000000);
rgb(281pt)=(1.000000,0.624000,0.000000);
rgb(282pt)=(1.000000,0.628000,0.000000);
rgb(283pt)=(1.000000,0.632000,0.000000);
rgb(284pt)=(1.000000,0.636000,0.000000);
rgb(285pt)=(1.000000,0.640000,0.000000);
rgb(286pt)=(1.000000,0.644000,0.000000);
rgb(287pt)=(1.000000,0.648000,0.000000);
rgb(288pt)=(1.000000,0.652000,0.000000);
rgb(289pt)=(1.000000,0.656000,0.000000);
rgb(290pt)=(1.000000,0.660000,0.000000);
rgb(291pt)=(1.000000,0.664000,0.000000);
rgb(292pt)=(1.000000,0.668000,0.000000);
rgb(293pt)=(1.000000,0.672000,0.000000);
rgb(294pt)=(1.000000,0.676000,0.000000);
rgb(295pt)=(1.000000,0.680000,0.000000);
rgb(296pt)=(1.000000,0.684000,0.000000);
rgb(297pt)=(1.000000,0.688000,0.000000);
rgb(298pt)=(1.000000,0.692000,0.000000);
rgb(299pt)=(1.000000,0.696000,0.000000);
rgb(300pt)=(1.000000,0.700000,0.000000);
rgb(301pt)=(1.000000,0.704000,0.000000);
rgb(302pt)=(1.000000,0.708000,0.000000);
rgb(303pt)=(1.000000,0.712000,0.000000);
rgb(304pt)=(1.000000,0.716000,0.000000);
rgb(305pt)=(1.000000,0.720000,0.000000);
rgb(306pt)=(1.000000,0.724000,0.000000);
rgb(307pt)=(1.000000,0.728000,0.000000);
rgb(308pt)=(1.000000,0.732000,0.000000);
rgb(309pt)=(1.000000,0.736000,0.000000);
rgb(310pt)=(1.000000,0.740000,0.000000);
rgb(311pt)=(1.000000,0.744000,0.000000);
rgb(312pt)=(1.000000,0.748000,0.000000);
rgb(313pt)=(1.000000,0.752000,0.000000);
rgb(314pt)=(1.000000,0.756000,0.000000);
rgb(315pt)=(1.000000,0.760000,0.000000);
rgb(316pt)=(1.000000,0.764000,0.000000);
rgb(317pt)=(1.000000,0.768000,0.000000);
rgb(318pt)=(1.000000,0.772000,0.000000);
rgb(319pt)=(1.000000,0.776000,0.000000);
rgb(320pt)=(1.000000,0.780000,0.000000);
rgb(321pt)=(1.000000,0.784000,0.000000);
rgb(322pt)=(1.000000,0.788000,0.000000);
rgb(323pt)=(1.000000,0.792000,0.000000);
rgb(324pt)=(1.000000,0.796000,0.000000);
rgb(325pt)=(1.000000,0.800000,0.000000);
rgb(326pt)=(1.000000,0.804000,0.000000);
rgb(327pt)=(1.000000,0.808000,0.000000);
rgb(328pt)=(1.000000,0.812000,0.000000);
rgb(329pt)=(1.000000,0.816000,0.000000);
rgb(330pt)=(1.000000,0.820000,0.000000);
rgb(331pt)=(1.000000,0.824000,0.000000);
rgb(332pt)=(1.000000,0.828000,0.000000);
rgb(333pt)=(1.000000,0.832000,0.000000);
rgb(334pt)=(1.000000,0.836000,0.000000);
rgb(335pt)=(1.000000,0.840000,0.000000);
rgb(336pt)=(1.000000,0.844000,0.000000);
rgb(337pt)=(1.000000,0.848000,0.000000);
rgb(338pt)=(1.000000,0.852000,0.000000);
rgb(339pt)=(1.000000,0.856000,0.000000);
rgb(340pt)=(1.000000,0.860000,0.000000);
rgb(341pt)=(1.000000,0.864000,0.000000);
rgb(342pt)=(1.000000,0.868000,0.000000);
rgb(343pt)=(1.000000,0.872000,0.000000);
rgb(344pt)=(1.000000,0.876000,0.000000);
rgb(345pt)=(1.000000,0.880000,0.000000);
rgb(346pt)=(1.000000,0.884000,0.000000);
rgb(347pt)=(1.000000,0.888000,0.000000);
rgb(348pt)=(1.000000,0.892000,0.000000);
rgb(349pt)=(1.000000,0.896000,0.000000);
rgb(350pt)=(1.000000,0.900000,0.000000);
rgb(351pt)=(1.000000,0.904000,0.000000);
rgb(352pt)=(1.000000,0.908000,0.000000);
rgb(353pt)=(1.000000,0.912000,0.000000);
rgb(354pt)=(1.000000,0.916000,0.000000);
rgb(355pt)=(1.000000,0.920000,0.000000);
rgb(356pt)=(1.000000,0.924000,0.000000);
rgb(357pt)=(1.000000,0.928000,0.000000);
rgb(358pt)=(1.000000,0.932000,0.000000);
rgb(359pt)=(1.000000,0.936000,0.000000);
rgb(360pt)=(1.000000,0.940000,0.000000);
rgb(361pt)=(1.000000,0.944000,0.000000);
rgb(362pt)=(1.000000,0.948000,0.000000);
rgb(363pt)=(1.000000,0.952000,0.000000);
rgb(364pt)=(1.000000,0.956000,0.000000);
rgb(365pt)=(1.000000,0.960000,0.000000);
rgb(366pt)=(1.000000,0.964000,0.000000);
rgb(367pt)=(1.000000,0.968000,0.000000);
rgb(368pt)=(1.000000,0.972000,0.000000);
rgb(369pt)=(1.000000,0.976000,0.000000);
rgb(370pt)=(1.000000,0.980000,0.000000);
rgb(371pt)=(1.000000,0.984000,0.000000);
rgb(372pt)=(1.000000,0.988000,0.000000);
rgb(373pt)=(1.000000,0.992000,0.000000);
rgb(374pt)=(1.000000,0.996000,0.000000);
rgb(375pt)=(1.000000,1.000000,0.000000);
rgb(376pt)=(0.996000,1.000000,0.004000);
rgb(377pt)=(0.992000,1.000000,0.008000);
rgb(378pt)=(0.988000,1.000000,0.012000);
rgb(379pt)=(0.984000,1.000000,0.016000);
rgb(380pt)=(0.980000,1.000000,0.020000);
rgb(381pt)=(0.976000,1.000000,0.024000);
rgb(382pt)=(0.972000,1.000000,0.028000);
rgb(383pt)=(0.968000,1.000000,0.032000);
rgb(384pt)=(0.964000,1.000000,0.036000);
rgb(385pt)=(0.960000,1.000000,0.040000);
rgb(386pt)=(0.956000,1.000000,0.044000);
rgb(387pt)=(0.952000,1.000000,0.048000);
rgb(388pt)=(0.948000,1.000000,0.052000);
rgb(389pt)=(0.944000,1.000000,0.056000);
rgb(390pt)=(0.940000,1.000000,0.060000);
rgb(391pt)=(0.936000,1.000000,0.064000);
rgb(392pt)=(0.932000,1.000000,0.068000);
rgb(393pt)=(0.928000,1.000000,0.072000);
rgb(394pt)=(0.924000,1.000000,0.076000);
rgb(395pt)=(0.920000,1.000000,0.080000);
rgb(396pt)=(0.916000,1.000000,0.084000);
rgb(397pt)=(0.912000,1.000000,0.088000);
rgb(398pt)=(0.908000,1.000000,0.092000);
rgb(399pt)=(0.904000,1.000000,0.096000);
rgb(400pt)=(0.900000,1.000000,0.100000);
rgb(401pt)=(0.896000,1.000000,0.104000);
rgb(402pt)=(0.892000,1.000000,0.108000);
rgb(403pt)=(0.888000,1.000000,0.112000);
rgb(404pt)=(0.884000,1.000000,0.116000);
rgb(405pt)=(0.880000,1.000000,0.120000);
rgb(406pt)=(0.876000,1.000000,0.124000);
rgb(407pt)=(0.872000,1.000000,0.128000);
rgb(408pt)=(0.868000,1.000000,0.132000);
rgb(409pt)=(0.864000,1.000000,0.136000);
rgb(410pt)=(0.860000,1.000000,0.140000);
rgb(411pt)=(0.856000,1.000000,0.144000);
rgb(412pt)=(0.852000,1.000000,0.148000);
rgb(413pt)=(0.848000,1.000000,0.152000);
rgb(414pt)=(0.844000,1.000000,0.156000);
rgb(415pt)=(0.840000,1.000000,0.160000);
rgb(416pt)=(0.836000,1.000000,0.164000);
rgb(417pt)=(0.832000,1.000000,0.168000);
rgb(418pt)=(0.828000,1.000000,0.172000);
rgb(419pt)=(0.824000,1.000000,0.176000);
rgb(420pt)=(0.820000,1.000000,0.180000);
rgb(421pt)=(0.816000,1.000000,0.184000);
rgb(422pt)=(0.812000,1.000000,0.188000);
rgb(423pt)=(0.808000,1.000000,0.192000);
rgb(424pt)=(0.804000,1.000000,0.196000);
rgb(425pt)=(0.800000,1.000000,0.200000);
rgb(426pt)=(0.796000,1.000000,0.204000);
rgb(427pt)=(0.792000,1.000000,0.208000);
rgb(428pt)=(0.788000,1.000000,0.212000);
rgb(429pt)=(0.784000,1.000000,0.216000);
rgb(430pt)=(0.780000,1.000000,0.220000);
rgb(431pt)=(0.776000,1.000000,0.224000);
rgb(432pt)=(0.772000,1.000000,0.228000);
rgb(433pt)=(0.768000,1.000000,0.232000);
rgb(434pt)=(0.764000,1.000000,0.236000);
rgb(435pt)=(0.760000,1.000000,0.240000);
rgb(436pt)=(0.756000,1.000000,0.244000);
rgb(437pt)=(0.752000,1.000000,0.248000);
rgb(438pt)=(0.748000,1.000000,0.252000);
rgb(439pt)=(0.744000,1.000000,0.256000);
rgb(440pt)=(0.740000,1.000000,0.260000);
rgb(441pt)=(0.736000,1.000000,0.264000);
rgb(442pt)=(0.732000,1.000000,0.268000);
rgb(443pt)=(0.728000,1.000000,0.272000);
rgb(444pt)=(0.724000,1.000000,0.276000);
rgb(445pt)=(0.720000,1.000000,0.280000);
rgb(446pt)=(0.716000,1.000000,0.284000);
rgb(447pt)=(0.712000,1.000000,0.288000);
rgb(448pt)=(0.708000,1.000000,0.292000);
rgb(449pt)=(0.704000,1.000000,0.296000);
rgb(450pt)=(0.700000,1.000000,0.300000);
rgb(451pt)=(0.696000,1.000000,0.304000);
rgb(452pt)=(0.692000,1.000000,0.308000);
rgb(453pt)=(0.688000,1.000000,0.312000);
rgb(454pt)=(0.684000,1.000000,0.316000);
rgb(455pt)=(0.680000,1.000000,0.320000);
rgb(456pt)=(0.676000,1.000000,0.324000);
rgb(457pt)=(0.672000,1.000000,0.328000);
rgb(458pt)=(0.668000,1.000000,0.332000);
rgb(459pt)=(0.664000,1.000000,0.336000);
rgb(460pt)=(0.660000,1.000000,0.340000);
rgb(461pt)=(0.656000,1.000000,0.344000);
rgb(462pt)=(0.652000,1.000000,0.348000);
rgb(463pt)=(0.648000,1.000000,0.352000);
rgb(464pt)=(0.644000,1.000000,0.356000);
rgb(465pt)=(0.640000,1.000000,0.360000);
rgb(466pt)=(0.636000,1.000000,0.364000);
rgb(467pt)=(0.632000,1.000000,0.368000);
rgb(468pt)=(0.628000,1.000000,0.372000);
rgb(469pt)=(0.624000,1.000000,0.376000);
rgb(470pt)=(0.620000,1.000000,0.380000);
rgb(471pt)=(0.616000,1.000000,0.384000);
rgb(472pt)=(0.612000,1.000000,0.388000);
rgb(473pt)=(0.608000,1.000000,0.392000);
rgb(474pt)=(0.604000,1.000000,0.396000);
rgb(475pt)=(0.600000,1.000000,0.400000);
rgb(476pt)=(0.596000,1.000000,0.404000);
rgb(477pt)=(0.592000,1.000000,0.408000);
rgb(478pt)=(0.588000,1.000000,0.412000);
rgb(479pt)=(0.584000,1.000000,0.416000);
rgb(480pt)=(0.580000,1.000000,0.420000);
rgb(481pt)=(0.576000,1.000000,0.424000);
rgb(482pt)=(0.572000,1.000000,0.428000);
rgb(483pt)=(0.568000,1.000000,0.432000);
rgb(484pt)=(0.564000,1.000000,0.436000);
rgb(485pt)=(0.560000,1.000000,0.440000);
rgb(486pt)=(0.556000,1.000000,0.444000);
rgb(487pt)=(0.552000,1.000000,0.448000);
rgb(488pt)=(0.548000,1.000000,0.452000);
rgb(489pt)=(0.544000,1.000000,0.456000);
rgb(490pt)=(0.540000,1.000000,0.460000);
rgb(491pt)=(0.536000,1.000000,0.464000);
rgb(492pt)=(0.532000,1.000000,0.468000);
rgb(493pt)=(0.528000,1.000000,0.472000);
rgb(494pt)=(0.524000,1.000000,0.476000);
rgb(495pt)=(0.520000,1.000000,0.480000);
rgb(496pt)=(0.516000,1.000000,0.484000);
rgb(497pt)=(0.512000,1.000000,0.488000);
rgb(498pt)=(0.508000,1.000000,0.492000);
rgb(499pt)=(0.504000,1.000000,0.496000);
rgb(500pt)=(0.500000,1.000000,0.500000);
rgb(501pt)=(0.496000,1.000000,0.504000);
rgb(502pt)=(0.492000,1.000000,0.508000);
rgb(503pt)=(0.488000,1.000000,0.512000);
rgb(504pt)=(0.484000,1.000000,0.516000);
rgb(505pt)=(0.480000,1.000000,0.520000);
rgb(506pt)=(0.476000,1.000000,0.524000);
rgb(507pt)=(0.472000,1.000000,0.528000);
rgb(508pt)=(0.468000,1.000000,0.532000);
rgb(509pt)=(0.464000,1.000000,0.536000);
rgb(510pt)=(0.460000,1.000000,0.540000);
rgb(511pt)=(0.456000,1.000000,0.544000);
rgb(512pt)=(0.452000,1.000000,0.548000);
rgb(513pt)=(0.448000,1.000000,0.552000);
rgb(514pt)=(0.444000,1.000000,0.556000);
rgb(515pt)=(0.440000,1.000000,0.560000);
rgb(516pt)=(0.436000,1.000000,0.564000);
rgb(517pt)=(0.432000,1.000000,0.568000);
rgb(518pt)=(0.428000,1.000000,0.572000);
rgb(519pt)=(0.424000,1.000000,0.576000);
rgb(520pt)=(0.420000,1.000000,0.580000);
rgb(521pt)=(0.416000,1.000000,0.584000);
rgb(522pt)=(0.412000,1.000000,0.588000);
rgb(523pt)=(0.408000,1.000000,0.592000);
rgb(524pt)=(0.404000,1.000000,0.596000);
rgb(525pt)=(0.400000,1.000000,0.600000);
rgb(526pt)=(0.396000,1.000000,0.604000);
rgb(527pt)=(0.392000,1.000000,0.608000);
rgb(528pt)=(0.388000,1.000000,0.612000);
rgb(529pt)=(0.384000,1.000000,0.616000);
rgb(530pt)=(0.380000,1.000000,0.620000);
rgb(531pt)=(0.376000,1.000000,0.624000);
rgb(532pt)=(0.372000,1.000000,0.628000);
rgb(533pt)=(0.368000,1.000000,0.632000);
rgb(534pt)=(0.364000,1.000000,0.636000);
rgb(535pt)=(0.360000,1.000000,0.640000);
rgb(536pt)=(0.356000,1.000000,0.644000);
rgb(537pt)=(0.352000,1.000000,0.648000);
rgb(538pt)=(0.348000,1.000000,0.652000);
rgb(539pt)=(0.344000,1.000000,0.656000);
rgb(540pt)=(0.340000,1.000000,0.660000);
rgb(541pt)=(0.336000,1.000000,0.664000);
rgb(542pt)=(0.332000,1.000000,0.668000);
rgb(543pt)=(0.328000,1.000000,0.672000);
rgb(544pt)=(0.324000,1.000000,0.676000);
rgb(545pt)=(0.320000,1.000000,0.680000);
rgb(546pt)=(0.316000,1.000000,0.684000);
rgb(547pt)=(0.312000,1.000000,0.688000);
rgb(548pt)=(0.308000,1.000000,0.692000);
rgb(549pt)=(0.304000,1.000000,0.696000);
rgb(550pt)=(0.300000,1.000000,0.700000);
rgb(551pt)=(0.296000,1.000000,0.704000);
rgb(552pt)=(0.292000,1.000000,0.708000);
rgb(553pt)=(0.288000,1.000000,0.712000);
rgb(554pt)=(0.284000,1.000000,0.716000);
rgb(555pt)=(0.280000,1.000000,0.720000);
rgb(556pt)=(0.276000,1.000000,0.724000);
rgb(557pt)=(0.272000,1.000000,0.728000);
rgb(558pt)=(0.268000,1.000000,0.732000);
rgb(559pt)=(0.264000,1.000000,0.736000);
rgb(560pt)=(0.260000,1.000000,0.740000);
rgb(561pt)=(0.256000,1.000000,0.744000);
rgb(562pt)=(0.252000,1.000000,0.748000);
rgb(563pt)=(0.248000,1.000000,0.752000);
rgb(564pt)=(0.244000,1.000000,0.756000);
rgb(565pt)=(0.240000,1.000000,0.760000);
rgb(566pt)=(0.236000,1.000000,0.764000);
rgb(567pt)=(0.232000,1.000000,0.768000);
rgb(568pt)=(0.228000,1.000000,0.772000);
rgb(569pt)=(0.224000,1.000000,0.776000);
rgb(570pt)=(0.220000,1.000000,0.780000);
rgb(571pt)=(0.216000,1.000000,0.784000);
rgb(572pt)=(0.212000,1.000000,0.788000);
rgb(573pt)=(0.208000,1.000000,0.792000);
rgb(574pt)=(0.204000,1.000000,0.796000);
rgb(575pt)=(0.200000,1.000000,0.800000);
rgb(576pt)=(0.196000,1.000000,0.804000);
rgb(577pt)=(0.192000,1.000000,0.808000);
rgb(578pt)=(0.188000,1.000000,0.812000);
rgb(579pt)=(0.184000,1.000000,0.816000);
rgb(580pt)=(0.180000,1.000000,0.820000);
rgb(581pt)=(0.176000,1.000000,0.824000);
rgb(582pt)=(0.172000,1.000000,0.828000);
rgb(583pt)=(0.168000,1.000000,0.832000);
rgb(584pt)=(0.164000,1.000000,0.836000);
rgb(585pt)=(0.160000,1.000000,0.840000);
rgb(586pt)=(0.156000,1.000000,0.844000);
rgb(587pt)=(0.152000,1.000000,0.848000);
rgb(588pt)=(0.148000,1.000000,0.852000);
rgb(589pt)=(0.144000,1.000000,0.856000);
rgb(590pt)=(0.140000,1.000000,0.860000);
rgb(591pt)=(0.136000,1.000000,0.864000);
rgb(592pt)=(0.132000,1.000000,0.868000);
rgb(593pt)=(0.128000,1.000000,0.872000);
rgb(594pt)=(0.124000,1.000000,0.876000);
rgb(595pt)=(0.120000,1.000000,0.880000);
rgb(596pt)=(0.116000,1.000000,0.884000);
rgb(597pt)=(0.112000,1.000000,0.888000);
rgb(598pt)=(0.108000,1.000000,0.892000);
rgb(599pt)=(0.104000,1.000000,0.896000);
rgb(600pt)=(0.100000,1.000000,0.900000);
rgb(601pt)=(0.096000,1.000000,0.904000);
rgb(602pt)=(0.092000,1.000000,0.908000);
rgb(603pt)=(0.088000,1.000000,0.912000);
rgb(604pt)=(0.084000,1.000000,0.916000);
rgb(605pt)=(0.080000,1.000000,0.920000);
rgb(606pt)=(0.076000,1.000000,0.924000);
rgb(607pt)=(0.072000,1.000000,0.928000);
rgb(608pt)=(0.068000,1.000000,0.932000);
rgb(609pt)=(0.064000,1.000000,0.936000);
rgb(610pt)=(0.060000,1.000000,0.940000);
rgb(611pt)=(0.056000,1.000000,0.944000);
rgb(612pt)=(0.052000,1.000000,0.948000);
rgb(613pt)=(0.048000,1.000000,0.952000);
rgb(614pt)=(0.044000,1.000000,0.956000);
rgb(615pt)=(0.040000,1.000000,0.960000);
rgb(616pt)=(0.036000,1.000000,0.964000);
rgb(617pt)=(0.032000,1.000000,0.968000);
rgb(618pt)=(0.028000,1.000000,0.972000);
rgb(619pt)=(0.024000,1.000000,0.976000);
rgb(620pt)=(0.020000,1.000000,0.980000);
rgb(621pt)=(0.016000,1.000000,0.984000);
rgb(622pt)=(0.012000,1.000000,0.988000);
rgb(623pt)=(0.008000,1.000000,0.992000);
rgb(624pt)=(0.004000,1.000000,0.996000);
rgb(625pt)=(0.000000,1.000000,1.000000);
rgb(626pt)=(0.000000,0.996000,1.000000);
rgb(627pt)=(0.000000,0.992000,1.000000);
rgb(628pt)=(0.000000,0.988000,1.000000);
rgb(629pt)=(0.000000,0.984000,1.000000);
rgb(630pt)=(0.000000,0.980000,1.000000);
rgb(631pt)=(0.000000,0.976000,1.000000);
rgb(632pt)=(0.000000,0.972000,1.000000);
rgb(633pt)=(0.000000,0.968000,1.000000);
rgb(634pt)=(0.000000,0.964000,1.000000);
rgb(635pt)=(0.000000,0.960000,1.000000);
rgb(636pt)=(0.000000,0.956000,1.000000);
rgb(637pt)=(0.000000,0.952000,1.000000);
rgb(638pt)=(0.000000,0.948000,1.000000);
rgb(639pt)=(0.000000,0.944000,1.000000);
rgb(640pt)=(0.000000,0.940000,1.000000);
rgb(641pt)=(0.000000,0.936000,1.000000);
rgb(642pt)=(0.000000,0.932000,1.000000);
rgb(643pt)=(0.000000,0.928000,1.000000);
rgb(644pt)=(0.000000,0.924000,1.000000);
rgb(645pt)=(0.000000,0.920000,1.000000);
rgb(646pt)=(0.000000,0.916000,1.000000);
rgb(647pt)=(0.000000,0.912000,1.000000);
rgb(648pt)=(0.000000,0.908000,1.000000);
rgb(649pt)=(0.000000,0.904000,1.000000);
rgb(650pt)=(0.000000,0.900000,1.000000);
rgb(651pt)=(0.000000,0.896000,1.000000);
rgb(652pt)=(0.000000,0.892000,1.000000);
rgb(653pt)=(0.000000,0.888000,1.000000);
rgb(654pt)=(0.000000,0.884000,1.000000);
rgb(655pt)=(0.000000,0.880000,1.000000);
rgb(656pt)=(0.000000,0.876000,1.000000);
rgb(657pt)=(0.000000,0.872000,1.000000);
rgb(658pt)=(0.000000,0.868000,1.000000);
rgb(659pt)=(0.000000,0.864000,1.000000);
rgb(660pt)=(0.000000,0.860000,1.000000);
rgb(661pt)=(0.000000,0.856000,1.000000);
rgb(662pt)=(0.000000,0.852000,1.000000);
rgb(663pt)=(0.000000,0.848000,1.000000);
rgb(664pt)=(0.000000,0.844000,1.000000);
rgb(665pt)=(0.000000,0.840000,1.000000);
rgb(666pt)=(0.000000,0.836000,1.000000);
rgb(667pt)=(0.000000,0.832000,1.000000);
rgb(668pt)=(0.000000,0.828000,1.000000);
rgb(669pt)=(0.000000,0.824000,1.000000);
rgb(670pt)=(0.000000,0.820000,1.000000);
rgb(671pt)=(0.000000,0.816000,1.000000);
rgb(672pt)=(0.000000,0.812000,1.000000);
rgb(673pt)=(0.000000,0.808000,1.000000);
rgb(674pt)=(0.000000,0.804000,1.000000);
rgb(675pt)=(0.000000,0.800000,1.000000);
rgb(676pt)=(0.000000,0.796000,1.000000);
rgb(677pt)=(0.000000,0.792000,1.000000);
rgb(678pt)=(0.000000,0.788000,1.000000);
rgb(679pt)=(0.000000,0.784000,1.000000);
rgb(680pt)=(0.000000,0.780000,1.000000);
rgb(681pt)=(0.000000,0.776000,1.000000);
rgb(682pt)=(0.000000,0.772000,1.000000);
rgb(683pt)=(0.000000,0.768000,1.000000);
rgb(684pt)=(0.000000,0.764000,1.000000);
rgb(685pt)=(0.000000,0.760000,1.000000);
rgb(686pt)=(0.000000,0.756000,1.000000);
rgb(687pt)=(0.000000,0.752000,1.000000);
rgb(688pt)=(0.000000,0.748000,1.000000);
rgb(689pt)=(0.000000,0.744000,1.000000);
rgb(690pt)=(0.000000,0.740000,1.000000);
rgb(691pt)=(0.000000,0.736000,1.000000);
rgb(692pt)=(0.000000,0.732000,1.000000);
rgb(693pt)=(0.000000,0.728000,1.000000);
rgb(694pt)=(0.000000,0.724000,1.000000);
rgb(695pt)=(0.000000,0.720000,1.000000);
rgb(696pt)=(0.000000,0.716000,1.000000);
rgb(697pt)=(0.000000,0.712000,1.000000);
rgb(698pt)=(0.000000,0.708000,1.000000);
rgb(699pt)=(0.000000,0.704000,1.000000);
rgb(700pt)=(0.000000,0.700000,1.000000);
rgb(701pt)=(0.000000,0.696000,1.000000);
rgb(702pt)=(0.000000,0.692000,1.000000);
rgb(703pt)=(0.000000,0.688000,1.000000);
rgb(704pt)=(0.000000,0.684000,1.000000);
rgb(705pt)=(0.000000,0.680000,1.000000);
rgb(706pt)=(0.000000,0.676000,1.000000);
rgb(707pt)=(0.000000,0.672000,1.000000);
rgb(708pt)=(0.000000,0.668000,1.000000);
rgb(709pt)=(0.000000,0.664000,1.000000);
rgb(710pt)=(0.000000,0.660000,1.000000);
rgb(711pt)=(0.000000,0.656000,1.000000);
rgb(712pt)=(0.000000,0.652000,1.000000);
rgb(713pt)=(0.000000,0.648000,1.000000);
rgb(714pt)=(0.000000,0.644000,1.000000);
rgb(715pt)=(0.000000,0.640000,1.000000);
rgb(716pt)=(0.000000,0.636000,1.000000);
rgb(717pt)=(0.000000,0.632000,1.000000);
rgb(718pt)=(0.000000,0.628000,1.000000);
rgb(719pt)=(0.000000,0.624000,1.000000);
rgb(720pt)=(0.000000,0.620000,1.000000);
rgb(721pt)=(0.000000,0.616000,1.000000);
rgb(722pt)=(0.000000,0.612000,1.000000);
rgb(723pt)=(0.000000,0.608000,1.000000);
rgb(724pt)=(0.000000,0.604000,1.000000);
rgb(725pt)=(0.000000,0.600000,1.000000);
rgb(726pt)=(0.000000,0.596000,1.000000);
rgb(727pt)=(0.000000,0.592000,1.000000);
rgb(728pt)=(0.000000,0.588000,1.000000);
rgb(729pt)=(0.000000,0.584000,1.000000);
rgb(730pt)=(0.000000,0.580000,1.000000);
rgb(731pt)=(0.000000,0.576000,1.000000);
rgb(732pt)=(0.000000,0.572000,1.000000);
rgb(733pt)=(0.000000,0.568000,1.000000);
rgb(734pt)=(0.000000,0.564000,1.000000);
rgb(735pt)=(0.000000,0.560000,1.000000);
rgb(736pt)=(0.000000,0.556000,1.000000);
rgb(737pt)=(0.000000,0.552000,1.000000);
rgb(738pt)=(0.000000,0.548000,1.000000);
rgb(739pt)=(0.000000,0.544000,1.000000);
rgb(740pt)=(0.000000,0.540000,1.000000);
rgb(741pt)=(0.000000,0.536000,1.000000);
rgb(742pt)=(0.000000,0.532000,1.000000);
rgb(743pt)=(0.000000,0.528000,1.000000);
rgb(744pt)=(0.000000,0.524000,1.000000);
rgb(745pt)=(0.000000,0.520000,1.000000);
rgb(746pt)=(0.000000,0.516000,1.000000);
rgb(747pt)=(0.000000,0.512000,1.000000);
rgb(748pt)=(0.000000,0.508000,1.000000);
rgb(749pt)=(0.000000,0.504000,1.000000);
rgb(750pt)=(0.000000,0.500000,1.000000);
rgb(751pt)=(0.000000,0.496000,1.000000);
rgb(752pt)=(0.000000,0.492000,1.000000);
rgb(753pt)=(0.000000,0.488000,1.000000);
rgb(754pt)=(0.000000,0.484000,1.000000);
rgb(755pt)=(0.000000,0.480000,1.000000);
rgb(756pt)=(0.000000,0.476000,1.000000);
rgb(757pt)=(0.000000,0.472000,1.000000);
rgb(758pt)=(0.000000,0.468000,1.000000);
rgb(759pt)=(0.000000,0.464000,1.000000);
rgb(760pt)=(0.000000,0.460000,1.000000);
rgb(761pt)=(0.000000,0.456000,1.000000);
rgb(762pt)=(0.000000,0.452000,1.000000);
rgb(763pt)=(0.000000,0.448000,1.000000);
rgb(764pt)=(0.000000,0.444000,1.000000);
rgb(765pt)=(0.000000,0.440000,1.000000);
rgb(766pt)=(0.000000,0.436000,1.000000);
rgb(767pt)=(0.000000,0.432000,1.000000);
rgb(768pt)=(0.000000,0.428000,1.000000);
rgb(769pt)=(0.000000,0.424000,1.000000);
rgb(770pt)=(0.000000,0.420000,1.000000);
rgb(771pt)=(0.000000,0.416000,1.000000);
rgb(772pt)=(0.000000,0.412000,1.000000);
rgb(773pt)=(0.000000,0.408000,1.000000);
rgb(774pt)=(0.000000,0.404000,1.000000);
rgb(775pt)=(0.000000,0.400000,1.000000);
rgb(776pt)=(0.000000,0.396000,1.000000);
rgb(777pt)=(0.000000,0.392000,1.000000);
rgb(778pt)=(0.000000,0.388000,1.000000);
rgb(779pt)=(0.000000,0.384000,1.000000);
rgb(780pt)=(0.000000,0.380000,1.000000);
rgb(781pt)=(0.000000,0.376000,1.000000);
rgb(782pt)=(0.000000,0.372000,1.000000);
rgb(783pt)=(0.000000,0.368000,1.000000);
rgb(784pt)=(0.000000,0.364000,1.000000);
rgb(785pt)=(0.000000,0.360000,1.000000);
rgb(786pt)=(0.000000,0.356000,1.000000);
rgb(787pt)=(0.000000,0.352000,1.000000);
rgb(788pt)=(0.000000,0.348000,1.000000);
rgb(789pt)=(0.000000,0.344000,1.000000);
rgb(790pt)=(0.000000,0.340000,1.000000);
rgb(791pt)=(0.000000,0.336000,1.000000);
rgb(792pt)=(0.000000,0.332000,1.000000);
rgb(793pt)=(0.000000,0.328000,1.000000);
rgb(794pt)=(0.000000,0.324000,1.000000);
rgb(795pt)=(0.000000,0.320000,1.000000);
rgb(796pt)=(0.000000,0.316000,1.000000);
rgb(797pt)=(0.000000,0.312000,1.000000);
rgb(798pt)=(0.000000,0.308000,1.000000);
rgb(799pt)=(0.000000,0.304000,1.000000);
rgb(800pt)=(0.000000,0.300000,1.000000);
rgb(801pt)=(0.000000,0.296000,1.000000);
rgb(802pt)=(0.000000,0.292000,1.000000);
rgb(803pt)=(0.000000,0.288000,1.000000);
rgb(804pt)=(0.000000,0.284000,1.000000);
rgb(805pt)=(0.000000,0.280000,1.000000);
rgb(806pt)=(0.000000,0.276000,1.000000);
rgb(807pt)=(0.000000,0.272000,1.000000);
rgb(808pt)=(0.000000,0.268000,1.000000);
rgb(809pt)=(0.000000,0.264000,1.000000);
rgb(810pt)=(0.000000,0.260000,1.000000);
rgb(811pt)=(0.000000,0.256000,1.000000);
rgb(812pt)=(0.000000,0.252000,1.000000);
rgb(813pt)=(0.000000,0.248000,1.000000);
rgb(814pt)=(0.000000,0.244000,1.000000);
rgb(815pt)=(0.000000,0.240000,1.000000);
rgb(816pt)=(0.000000,0.236000,1.000000);
rgb(817pt)=(0.000000,0.232000,1.000000);
rgb(818pt)=(0.000000,0.228000,1.000000);
rgb(819pt)=(0.000000,0.224000,1.000000);
rgb(820pt)=(0.000000,0.220000,1.000000);
rgb(821pt)=(0.000000,0.216000,1.000000);
rgb(822pt)=(0.000000,0.212000,1.000000);
rgb(823pt)=(0.000000,0.208000,1.000000);
rgb(824pt)=(0.000000,0.204000,1.000000);
rgb(825pt)=(0.000000,0.200000,1.000000);
rgb(826pt)=(0.000000,0.196000,1.000000);
rgb(827pt)=(0.000000,0.192000,1.000000);
rgb(828pt)=(0.000000,0.188000,1.000000);
rgb(829pt)=(0.000000,0.184000,1.000000);
rgb(830pt)=(0.000000,0.180000,1.000000);
rgb(831pt)=(0.000000,0.176000,1.000000);
rgb(832pt)=(0.000000,0.172000,1.000000);
rgb(833pt)=(0.000000,0.168000,1.000000);
rgb(834pt)=(0.000000,0.164000,1.000000);
rgb(835pt)=(0.000000,0.160000,1.000000);
rgb(836pt)=(0.000000,0.156000,1.000000);
rgb(837pt)=(0.000000,0.152000,1.000000);
rgb(838pt)=(0.000000,0.148000,1.000000);
rgb(839pt)=(0.000000,0.144000,1.000000);
rgb(840pt)=(0.000000,0.140000,1.000000);
rgb(841pt)=(0.000000,0.136000,1.000000);
rgb(842pt)=(0.000000,0.132000,1.000000);
rgb(843pt)=(0.000000,0.128000,1.000000);
rgb(844pt)=(0.000000,0.124000,1.000000);
rgb(845pt)=(0.000000,0.120000,1.000000);
rgb(846pt)=(0.000000,0.116000,1.000000);
rgb(847pt)=(0.000000,0.112000,1.000000);
rgb(848pt)=(0.000000,0.108000,1.000000);
rgb(849pt)=(0.000000,0.104000,1.000000);
rgb(850pt)=(0.000000,0.100000,1.000000);
rgb(851pt)=(0.000000,0.096000,1.000000);
rgb(852pt)=(0.000000,0.092000,1.000000);
rgb(853pt)=(0.000000,0.088000,1.000000);
rgb(854pt)=(0.000000,0.084000,1.000000);
rgb(855pt)=(0.000000,0.080000,1.000000);
rgb(856pt)=(0.000000,0.076000,1.000000);
rgb(857pt)=(0.000000,0.072000,1.000000);
rgb(858pt)=(0.000000,0.068000,1.000000);
rgb(859pt)=(0.000000,0.064000,1.000000);
rgb(860pt)=(0.000000,0.060000,1.000000);
rgb(861pt)=(0.000000,0.056000,1.000000);
rgb(862pt)=(0.000000,0.052000,1.000000);
rgb(863pt)=(0.000000,0.048000,1.000000);
rgb(864pt)=(0.000000,0.044000,1.000000);
rgb(865pt)=(0.000000,0.040000,1.000000);
rgb(866pt)=(0.000000,0.036000,1.000000);
rgb(867pt)=(0.000000,0.032000,1.000000);
rgb(868pt)=(0.000000,0.028000,1.000000);
rgb(869pt)=(0.000000,0.024000,1.000000);
rgb(870pt)=(0.000000,0.020000,1.000000);
rgb(871pt)=(0.000000,0.016000,1.000000);
rgb(872pt)=(0.000000,0.012000,1.000000);
rgb(873pt)=(0.000000,0.008000,1.000000);
rgb(874pt)=(0.000000,0.004000,1.000000);
rgb(875pt)=(0.000000,0.000000,1.000000);
rgb(876pt)=(0.000000,0.000000,0.996000);
rgb(877pt)=(0.000000,0.000000,0.992000);
rgb(878pt)=(0.000000,0.000000,0.988000);
rgb(879pt)=(0.000000,0.000000,0.984000);
rgb(880pt)=(0.000000,0.000000,0.980000);
rgb(881pt)=(0.000000,0.000000,0.976000);
rgb(882pt)=(0.000000,0.000000,0.972000);
rgb(883pt)=(0.000000,0.000000,0.968000);
rgb(884pt)=(0.000000,0.000000,0.964000);
rgb(885pt)=(0.000000,0.000000,0.960000);
rgb(886pt)=(0.000000,0.000000,0.956000);
rgb(887pt)=(0.000000,0.000000,0.952000);
rgb(888pt)=(0.000000,0.000000,0.948000);
rgb(889pt)=(0.000000,0.000000,0.944000);
rgb(890pt)=(0.000000,0.000000,0.940000);
rgb(891pt)=(0.000000,0.000000,0.936000);
rgb(892pt)=(0.000000,0.000000,0.932000);
rgb(893pt)=(0.000000,0.000000,0.928000);
rgb(894pt)=(0.000000,0.000000,0.924000);
rgb(895pt)=(0.000000,0.000000,0.920000);
rgb(896pt)=(0.000000,0.000000,0.916000);
rgb(897pt)=(0.000000,0.000000,0.912000);
rgb(898pt)=(0.000000,0.000000,0.908000);
rgb(899pt)=(0.000000,0.000000,0.904000);
rgb(900pt)=(0.000000,0.000000,0.900000);
rgb(901pt)=(0.000000,0.000000,0.896000);
rgb(902pt)=(0.000000,0.000000,0.892000);
rgb(903pt)=(0.000000,0.000000,0.888000);
rgb(904pt)=(0.000000,0.000000,0.884000);
rgb(905pt)=(0.000000,0.000000,0.880000);
rgb(906pt)=(0.000000,0.000000,0.876000);
rgb(907pt)=(0.000000,0.000000,0.872000);
rgb(908pt)=(0.000000,0.000000,0.868000);
rgb(909pt)=(0.000000,0.000000,0.864000);
rgb(910pt)=(0.000000,0.000000,0.860000);
rgb(911pt)=(0.000000,0.000000,0.856000);
rgb(912pt)=(0.000000,0.000000,0.852000);
rgb(913pt)=(0.000000,0.000000,0.848000);
rgb(914pt)=(0.000000,0.000000,0.844000);
rgb(915pt)=(0.000000,0.000000,0.840000);
rgb(916pt)=(0.000000,0.000000,0.836000);
rgb(917pt)=(0.000000,0.000000,0.832000);
rgb(918pt)=(0.000000,0.000000,0.828000);
rgb(919pt)=(0.000000,0.000000,0.824000);
rgb(920pt)=(0.000000,0.000000,0.820000);
rgb(921pt)=(0.000000,0.000000,0.816000);
rgb(922pt)=(0.000000,0.000000,0.812000);
rgb(923pt)=(0.000000,0.000000,0.808000);
rgb(924pt)=(0.000000,0.000000,0.804000);
rgb(925pt)=(0.000000,0.000000,0.800000);
rgb(926pt)=(0.000000,0.000000,0.796000);
rgb(927pt)=(0.000000,0.000000,0.792000);
rgb(928pt)=(0.000000,0.000000,0.788000);
rgb(929pt)=(0.000000,0.000000,0.784000);
rgb(930pt)=(0.000000,0.000000,0.780000);
rgb(931pt)=(0.000000,0.000000,0.776000);
rgb(932pt)=(0.000000,0.000000,0.772000);
rgb(933pt)=(0.000000,0.000000,0.768000);
rgb(934pt)=(0.000000,0.000000,0.764000);
rgb(935pt)=(0.000000,0.000000,0.760000);
rgb(936pt)=(0.000000,0.000000,0.756000);
rgb(937pt)=(0.000000,0.000000,0.752000);
rgb(938pt)=(0.000000,0.000000,0.748000);
rgb(939pt)=(0.000000,0.000000,0.744000);
rgb(940pt)=(0.000000,0.000000,0.740000);
rgb(941pt)=(0.000000,0.000000,0.736000);
rgb(942pt)=(0.000000,0.000000,0.732000);
rgb(943pt)=(0.000000,0.000000,0.728000);
rgb(944pt)=(0.000000,0.000000,0.724000);
rgb(945pt)=(0.000000,0.000000,0.720000);
rgb(946pt)=(0.000000,0.000000,0.716000);
rgb(947pt)=(0.000000,0.000000,0.712000);
rgb(948pt)=(0.000000,0.000000,0.708000);
rgb(949pt)=(0.000000,0.000000,0.704000);
rgb(950pt)=(0.000000,0.000000,0.700000);
rgb(951pt)=(0.000000,0.000000,0.696000);
rgb(952pt)=(0.000000,0.000000,0.692000);
rgb(953pt)=(0.000000,0.000000,0.688000);
rgb(954pt)=(0.000000,0.000000,0.684000);
rgb(955pt)=(0.000000,0.000000,0.680000);
rgb(956pt)=(0.000000,0.000000,0.676000);
rgb(957pt)=(0.000000,0.000000,0.672000);
rgb(958pt)=(0.000000,0.000000,0.668000);
rgb(959pt)=(0.000000,0.000000,0.664000);
rgb(960pt)=(0.000000,0.000000,0.660000);
rgb(961pt)=(0.000000,0.000000,0.656000);
rgb(962pt)=(0.000000,0.000000,0.652000);
rgb(963pt)=(0.000000,0.000000,0.648000);
rgb(964pt)=(0.000000,0.000000,0.644000);
rgb(965pt)=(0.000000,0.000000,0.640000);
rgb(966pt)=(0.000000,0.000000,0.636000);
rgb(967pt)=(0.000000,0.000000,0.632000);
rgb(968pt)=(0.000000,0.000000,0.628000);
rgb(969pt)=(0.000000,0.000000,0.624000);
rgb(970pt)=(0.000000,0.000000,0.620000);
rgb(971pt)=(0.000000,0.000000,0.616000);
rgb(972pt)=(0.000000,0.000000,0.612000);
rgb(973pt)=(0.000000,0.000000,0.608000);
rgb(974pt)=(0.000000,0.000000,0.604000);
rgb(975pt)=(0.000000,0.000000,0.600000);
rgb(976pt)=(0.000000,0.000000,0.596000);
rgb(977pt)=(0.000000,0.000000,0.592000);
rgb(978pt)=(0.000000,0.000000,0.588000);
rgb(979pt)=(0.000000,0.000000,0.584000);
rgb(980pt)=(0.000000,0.000000,0.580000);
rgb(981pt)=(0.000000,0.000000,0.576000);
rgb(982pt)=(0.000000,0.000000,0.572000);
rgb(983pt)=(0.000000,0.000000,0.568000);
rgb(984pt)=(0.000000,0.000000,0.564000);
rgb(985pt)=(0.000000,0.000000,0.560000);
rgb(986pt)=(0.000000,0.000000,0.556000);
rgb(987pt)=(0.000000,0.000000,0.552000);
rgb(988pt)=(0.000000,0.000000,0.548000);
rgb(989pt)=(0.000000,0.000000,0.544000);
rgb(990pt)=(0.000000,0.000000,0.540000);
rgb(991pt)=(0.000000,0.000000,0.536000);
rgb(992pt)=(0.000000,0.000000,0.532000);
rgb(993pt)=(0.000000,0.000000,0.528000);
rgb(994pt)=(0.000000,0.000000,0.524000);
rgb(995pt)=(0.000000,0.000000,0.520000);
rgb(996pt)=(0.000000,0.000000,0.516000);
rgb(997pt)=(0.000000,0.000000,0.512000);
rgb(998pt)=(0.000000,0.000000,0.508000);
rgb(999pt)=(0.000000,0.000000,0.504000);
}}
